Is Support Set Diversity Necessary for Meta-Learning?

Meta-learning is a popular framework for learning with limited data in which an algorithm is produced by training over multiple few-shot learning tasks. For classification problems, these tasks are typically constructed by sampling a small number of support and query examples from a subset of the classes. While conventional wisdom is that task diversity should improve the performance of meta-learning, in this work we find evidence to the contrary: we propose a modification to traditional meta-learning approaches in which we keep the support sets fixed across tasks, thus reducing task diversity. Surprisingly, we find that not only does this modification not result in adverse effects, it almost always improves the performance for a variety of datasets and meta-learning methods. We also provide several initial analyses to understand this phenomenon. Our work serves to: (i) more closely investigate the effect of support set construction for the problem of meta-learning, and (ii) suggest a simple, general, and competitive baseline for few-shot learning.

==> sections/analysis.tex <==


% \subsection{Analysis}

% \begin{equation}
%     \frac{1}{T} \sum_{t=1}^{T} \frac{1}{n} \sum_{i=1}^n l((D c_t)^Tx_{ti}, y_{ti})
% \end{equation}


% $u_t = D c_t$, where $D \in \Real^{d \times K}$, $c_t \in \Real^K$.



% Possible candidates of $l: \Real \times \Real \rightarrow \Real$:
% \begin{itemize}
% \item Regression: $l(a,b)=(a-b)^2$
% \item 0-1 Classification: $\I(a \neq b)$
% \end{itemize}


% For regression, each task is a $(D, c_t)$ pair where we specify the distribution of the covariates $X$ as below and $y = (Dc_t)^T X + \epsilon$ whereas for classification, each task is a $(D, c_t)$ pair, we need to specify the distribution of the covariates $X$ as below and $y = \Sign{(u_t^Tx)}$.  


% Possible candidates of $X$ distribution for a task:
% \begin{itemize}
% \item uniform distribution over $S^{\sqrt{d}}_{d-1}$
% \item Gaussian distribution in $\Real^d$
% \end{itemize}

% Possible candidate for the distribution of $\epsilon$:
% \begin{itemize}
%     \item Gaussian distribution $\calN(0, \sigma^2 I)$.
% \end{itemize}

% The support set data of a task is represented as a $(X, y)$ pair, with $X \in \Real^{n \times d}$, $y \in \Real^n$.

% Option 1:
% Each task also has another query set dataset in the form $(X_q, y_q) \in \Real^{q \times d}, \Real^{q}$.

% Option 2:
% We use the formulation of The Benefit of Multitask Representation Learning, where there is no support/query set structure during training. 


% $K=5$
% $n=5, 10$
% $d=50$
% $q=25$

% ML vs FixML

% % Sampling Tasks for ML vs FixML
% U se a few fixed $\{X_1, X_2, ..., X_m\} \subseteq \{X_1, X_2, ..., X_M\}$
% Use a few fixed $\{c_1, c_2 \ldots  c_T\}$

% \begin{algorithm}
% \SetKwFunction{alg}{TaskSample}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Given $D$}
% \Output{$(X, y)$}
% \alg{$D$}:

% Sample $c_t$ \\
% Sample $X$ either according to the covariate distribution or uniformly from a collection of such matrices\\
% Let $y = XDc_t (+ \epsilon)$. \\
% Return $(X, y, c_t)$.
% \end{algorithm}


% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{Given $(X, y, c_t)$}

% $\hat{u}_t = D\hat{c}_t$ \\
% $\hat{c}_t = \arg\min_{c} \|XDc - y\|_2^2 = (D^TX^TXD)^{-1}D^TX^Ty$ \\
% $\E_{x} ((\hat{c}_t - c_t) D^T x)^2$ 

% \end{algorithm}


% For a specific task $(X, y)$, the post adaptation loss on the support set has the form:
% \begin{align*}
% &\norm{XD(D^TX^TXD)^{-1}D^TX^Ty - y}_2^2\\
% =& \; y^T (XD(D^TX^TXD)^{-1}D^TX^T - I)^T (XD(D^TX^TXD)^{-1}D^TX^T - I)y\\
% =&\; y^T (I - XD(D^TX^TXD)^{-1}D^TX^T)y \\
% =&\; \norm{y}_2^2 - (D^TX^Ty)^T(D^TX^TXD)^{-1}(D^TX^Ty)
% \end{align*}

% The derivative of this with respect to $D$ is:
% \begin{align*}
% \nabla_D =& -2X^Ty(\red{(D^TX^TXD)^{-1}(D^TX^Ty)})^T \\
% &\qquad + 2 X^TXD(\red{(D^TX^TXD)^{-1}(D^TX^Ty)})(\red{(D^TX^TXD)^{-1}(D^TX^Ty)})^T
% \end{align*}


% Alternatively, if we were to use regularization in the inner loop \ie then we optimize for $D$ using the following updates:
% \begin{align*}
% \hat{c} = \hat{c}(X,y,D) &= \arg\min_c\norm{XDc-y}_2^2 + \lambda \norm{c}^2_2 \\
% &= (D^TX^TXD + \lambda I)^{-1} D^T X^T y
% \\
% D &= D - \alpha \nabla_D \norm{XD\hat{c}(X,y,D) - y}^2
% \end{align*}

% Then, for a specific task $(X, y)$, the post adaptation loss on the support set has the form:

% \begin{align*}
% &\norm{XD(D^TX^TXD + \lambda I)^{-1}D^TX^Ty - y}_2^2\\
% =&\;  y^T (XD(D^TX^TXD+ \lambda I)^{-1}D^TX^T - I)^T (XD(D^TX^TXD+ \lambda I)^{-1}D^TX^T - I)y\\
% =& \; \norm{y}^2 -2 y^T XD(D^TX^TXD+ \lambda I)^{-1}D^TX^Ty \\
% & \qquad +y^TXD(D^TX^TXD+ \lambda I)^{-1}D^TX^T    XD(D^TX^TXD+ \lambda I)^{-1}D^TX^Ty
% \end{align*}


% From Woodburry Identity we know that:
% \begin{align*}
%   (D^TX^TXD+ \lambda I)^{-1} =& (D^TX^TXD)^{-1}(I - \lambda(D^TX^TXD + \lambda I)^{-1}) \\
%   =& \os{D^TX^T(XDD^TX^T + \lambda I)^{-1}y}
% \end{align*}


% \begin{align*}
% &\norm{XD(D^TX^TXD + \lambda I)^{-1}D^TX^Ty - y}_2^2\\
% =& \; \norm{y}^2 -2 y^T XD(D^TX^TXD+ \lambda I)^{-1}D^TX^Ty \\
% & \qquad +y^TXD(D^TX^TXD+ \lambda I)^{-1} (I - \lambda(D^TX^TXD + \lambda I)^{-1})D^TX^Ty \\
% =& \; \norm{y}^2 - (D^TX^Ty)(D^TX^TXD+ \lambda I)^{-1}(D^TX^Ty) \\
% & \qquad - \lambda (D^TX^Ty)(D^TX^TXD+ \lambda I)^{-2}(D^TX^Ty)
% \end{align*}

% Possible things to try:
% \begin{itemize}
% \item add randomness to y
% \item use a D whose K is greater than the true D.
% \item maybe add some corruption or wrong noise to y or X during training so that the training and test scenario does not match exactly
% \item Add noise to $D$ at test, causing some shift in the distribution of optimal predictor $Dc$ between train and test. 
% \end{itemize}



%     % A = X @ D # n x k
%     % A2 = X2 @ D # n2 x k
%     % AT = A.T # k x n
%     % A2T = A2.T # k x n2

%     % AAT = A @ A.T # n x n
%     % S = inv(AAT + (lambd * I)) # T_0   # n x n

%     % Sy = S @ y # n x 1
%     % XTSy = (X.T) @ Sy # t_1 (d x 1)
%     % c_solved = D.T @ XTSy # k x 1

%     % pred = A2 @ c_solved # n2 x 1
%     % err = (pred - y2) # t_2 (n2 x 1)
    
%     % ATSy = AT @ Sy # t_3 (k x 1)
%     % X2Terr = X2.T @ err  # t_4 d x 1
%     % A2Terr = A2T @ err # t_5
%     % SAA2Terr = S @ (A @ A2Terr)

%     % functionValue = (norm(err) ** 2)
%     % gradient = (2 * outer(X2Terr, ATSy))\
%     %         + (2 * outer(XTSy, A2Terr))\
%     %         - (2 * outer(X.T @ SAA2Terr, ATSy))\
%     %         - (2 * outer(XTSy, A.T @ SAA2Terr))

% % \begin{align*}
% % \nabla_D =& (\red{y^TXD (D^TX^TXD+ \lambda I)^{-1}} D^TX^T-y^T)XD(D^TX^TXD+ \lambda I)^{-1} \\
% % =& (\hat{c}^T  D^TX^TXD(D^TX^TXD+ \lambda I)^{-1}-\red{y^TXD(D^TX^TXD+ \lambda I)^{-1}}) \\
% % =& (\hat{c}^T   D^TX^TXD(D^TX^TXD+ \lambda I)^{-1} - \hat{c}^T)  \\
% % =& \hat{c}^T (D^TX^TXD(D^TX^TXD+ \lambda I)^{-1} - I)
% % \end{align*}



% \begin{align*}
% \min_D \frac{1}{|\calD|}\sum\limits_{((X_s, y_s), (X_q, y_q)) \in \calD} \norm{X_qDD^TX_s^T(X_sDD^TX_s^T + \lambda I)^{-1}y_s - y_q}_2^2
% \end{align*}


% We now compute the gradient of the above objective w.r.t. parameter $D$. For convenience we first define the following terms which determine the solution $\hat{c}$ and prediction $\hat{y}_q$ for the linear regression problem for each task (given $X_s,\; y_s$). 
% \begin{align*}
%     S &= (X_sDD^TX_s^T + \lambda I)^{-1} \nonumber \\ 
%     \hat{c} &= D^TX_s^TSy_s \nonumber \\
%     \hat{y}_q &= X_qD\hat{c}
% \end{align*}
% \begin{align}
%     \nabla_D &= 2 \red{X_q^T (\hat{y}_q - y_q)y_s^TSX_s}D   + 2\red{X_s^TSy_s (\hat{y}_q - y_q)^T X_q}D \nonumber \\
%     & \qquad  -2 X_s^T S X_s D D^T\red{X_q^T (\hat{y}_q - y_q)  y_s^TSX_s}D \; \nonumber \\
%     & \qquad  -2 \red{X_s^TSy_s  (\hat{y}_q - y_q)^TX_q}DD^TX_s^T SX_s D
% \end{align}
% Further, let $M \coloneqq X_q^T (\hat{y}_q - y_q)y_s^TSX_s$ be used to define a matrix $\in \Real^{d \times d}$. Then,
% \begin{align}
%     \nabla_D &= 2MD + 2M^TD - 2 X_s^T S X_s D D^TMD - 2M^TDD^TX_s^T SX_s D \nonumber \\
%     &= 2MD (I - X_s^T S X_s D D^T) + 2M^TD(I - D^TX_s^T SX_s D) \; 
% \end{align}


% \textit{Should we be looking at comparison of fix-ml and ml performance at their respective stationary points or the minimum over the entire trajectory? 
% }


% The expectation (over only query sets) for the fix-ml gradient is easier to compute. But its very hard to compute something like  $\E_R[R^{-1}]$ when we are computing the mean gradient w.r.t. the support set for the ml-gradient. 

% How can we reason about this? For the optimization side, we need to compute gradient bias $\mu$ for the fix-ml gradient. We also need to compute $\textrm{tr}(\E (\nabla_D - \E \nabla_D) (\nabla_D - \E \nabla_D)^T)$. 

% For generalization, may be we compute the uncentered gradient co-variance matrix $\bC \coloneqq \E \nabla_D \nabla_D^T$. Not sure if we can analytically derive $\bH$ though? 



% \red{Can FIX-ML be better than ML purely in terms of base distribution generalization?
% }

% To answer this question we need to first introduce some terms for the empirical error, true error and excess risk for both \fixml and \ml. We are learning the parameters of the algorithm $D$. We begin by defining the true error: 


% \begin{align*}
%     \calE(D, n_s, \lambda) = \E_{\tau} \E_{X_s, c_t | \tau} \norm{\hat{w}(D, X_s, c_t, \lambda) - w_t^*}^2 
% \end{align*}

% where we define our finite sample estimator $\hat{w}(D, X_s, c_t)$ as:

% \begin{align*}
%     \hat{w}(D, X_s, c_t, \lambda) = D^TX_s^T(X_sDD^TX_s^T + \lambda I)^{-1} \underbrace{(X_sD^*c_t)}_{y_s} 
% \end{align*}


% where $n_s$ is the number of support samples. In our case $X_s, c_t | \tau$. This is not needed for the re-formulation below but we use it for convenience. 


% \begin{align*}
%     \calE(D, n_s, \lambda) =  \E_{X_s} \E_{c_t}  \norm{\hat{w}(D, X_s, c_t, \lambda) - w_t^*}^2  = \E_{X_s} \E_{c_t}  \norm{\hat{w}(D, X_s, c_t, \lambda) - D^*c_t}^2 
% \end{align*}


% We can now define the true error w.r.t a particular support set $X_s$ as:


% \begin{align*}
%         \calE(D, n_s, \lambda, X_s) &=  \E_{c_t}  \norm{\hat{w}(D, X_s, c_t, \lambda) - w_t^*}^2 \\
%         \E_{X_s} \calE(D, n_s, \lambda, X_s) &= \calE(D, n_s, \lambda) 
% \end{align*}


% Similarly, we can define the empirical error which we refer to as the \ml objective and its biased version specific to a given support set $X_s$ which we refer to as \fixml objective. 



% \begin{align*}
%         \hat{\calE}\paren{D, \cbrck{X_{s,i}}_{i \in [N]},  \cbrck{c_j}_{j \in [N]}, \lambda} 
%         &=  \frac{1}{N^2} \sum_{i \in [N]}  \sum_{j \in [N]}   \norm{\hat{w}(D, X_{s,i}, c_{t,j}, \lambda) - D^*c_{t,j}}^2 \\
%         \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}}  &=  \frac{1}{N} \sum_{j \in [N]}  \norm{\hat{w}(D, X_{s}, c_{t,j}, \lambda) - D^*c_{t,i}}^2 \\
%         \E_{X_s \sim \hat{p}_\tau} \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda}  &=  \hat{\calE}\paren{D, \cbrck{X_{s,i}}_{i \in [N]},  \cbrck{c_j}_{j \in [N]}, \lambda} 
% \end{align*}


% The quantity we are interested in is the expected generalization gap for a given parameter $D$ of the algorithm (base learner). 

% \begin{align*}
%     & \calG(D, n_s, \lambda) = \E_{X_s,  \cbrck{c_j}_{j \in [N]}}\paren{\hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda} - \calE(D, n_s, \lambda)}^2 \\
%      & =   \E_{X_s,  \cbrck{c_j}_{j \in [N]}}\paren{\hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda} - \E_{X_s} \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda}}^2\\
%      & \qquad + \paren{\E_{X_s} \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda} - \calE(D, n_s, \lambda)}^2 \\
%      & = \E_{\cbrck{c_j}_{j \in [N]}} \brck{\V_{X_s} \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda}} + \V_{\cbrck{c_j}_{j \in [N]}} \underbrace{\brck{\E_{X_s} \hat{\calE}\paren{D, X_s,  \cbrck{c_j}_{j \in [N]}, \lambda}}}_{\approx \; \textrm{\red{\ml obj.}}} 
% \end{align*}



% We can re-write the excess risk in the following two ways for \fixml, where we have used the notion of generalization w.r.t. a particular $X_s$ :


% \begin{align*}
%     \hat{\calE}(D, X_s) - \calE(D) = \hat{\calE}(D, X_s) - \hat{\calE}(D) + \red{\hat{\calE}(D) -  \calE(D)} \\
%     \hat{\calE}(D, X_s) - \calE(D) = \red{\hat{\calE}(D, X_s) - \calE(D, X_s)} + \calE(D, X_s) -  \calE(D)
% \end{align*}



% \red{Reasoning about Base Class Generalization:}

% \underline{Expressivity}

% Are the algorithm's parameters express enough, such that there exists an optimal solution for the specific task in the scope of the Algorithm's parameters. For MAML, this can be an $\epsilon$ ball around the initialization. For subspace learning, this can be the size of the dictionary. 


% \underline{Inner loop Optimization}

% In the inner loop, $\hat{c}_t = f(D, X_{s, t})$ where $D$ is the algorithm parameters. First question is how well does $\hat{c}_t$ solve the inner loop. In most cases, this won't be an issue. 

% \underline{Task Specific Generalization}

% W.h.p. $\geq 1-\delta$ is the following true?

% $$
% \norm{f(D, X_{s, t}) - w_t} \leq \epsilon
% $$

% or in weaker terms:

% $$
% \E \norm{f(D, X_{s, t}) - w_t} \leq \epsilon
% $$







% % \[
% %   f = \|X\cdot D\cdot \mathrm{inv}(D^\top \cdot X^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top \cdot y-y\|_2^{2}
% % \]

% % gradient:
% % \[
% %   \frac{\partial f}{\partial D} = 2\cdot X^\top \cdot (X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top \cdot y-y)\cdot (y^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I}))-(2\cdot X^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top \cdot y\cdot ((y^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top +(-y)^\top )\cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I}))+2\cdot X^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top \cdot (X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top \cdot y-y)\cdot (y^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})))+2\cdot X^\top \cdot y\cdot ((y^\top \cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I})\cdot D^\top \cdot X^\top +(-y)^\top )\cdot X\cdot D\cdot \mathrm{inv}((X\cdot D)^\top \cdot X\cdot D+c\cdot \mathbb{I}))
% % \]
% % where
% % \begin{itemize}
% %   \item $D$ is a matrix
% %   \item $X$ is a matrix
% %   \item $c$ is a scalar
% %   \item $y$ is a vector
% % \end{itemize}




\section{Convex Case}

Here, we try to analyze whether \fixml performs better than ML when the true risk is a convex quadratic in the parameter $\theta$. For this, we consider meta-linear regression where the inner loop adaptation is done by a single step of SGD on the support set. 

% \begin{align*}
%     \calR(\theta;\tau, \alpha) &= \E_{X_s,\theta_\tau|\tau} \calL(\hat{\theta}(X_s, \theta_\tau, \theta, \alpha);\tau) \\
%     \hat{\theta}(X_s, \theta_\tau, \theta, \alpha) &= \theta - \alpha \nabla_{\theta} \brck{ (\theta - \theta_\tau)^TX_s^TX_s(\theta - \theta_\tau)} \\
%     \calL(\cdot; \tau) &= \E_{\bx, y | \tau} \norm{\angleproduct{\bx, \cdot} - y}
% \end{align*}


Let's say we are given $M$ tasks, each with $n$ support and $n$ query samples, with the following structure:

\begin{align*}
\bx \sim \calN(\mathbf{0}, \Sigma_\tau) \qquad \Sigma_\tau = \bV \textrm{diag}(\btheta_\tau) \bV^T \qquad  \bepsilon \sim \calN(\mathbf{0}, \sigma^2_\tau \bI) \qquad y = \bx^T \btheta_\tau + \epsilon  
\end{align*}


\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{images/gm.png}
    \caption{Graphical Model for the meta-linear regression task distribution.}
    \label{fig:gm}
\end{figure}

% The assumptions we encode with the above Structural Causal Model are: $\epsilon_\tau \perp \theta_\tau | \tau$. 


\underline{Meta-Learning:}
If the task distribution is given by $p(\tau)$ we define the true risk for parameter $\eta$ on task $\tau$ as $\calR(\eta; \tau)$:
\begin{align*}
    \calR(\eta; \tau) &= \E_{X, y | \tau} \frac{1}{2} \norm{X\eta - y}_2^2 = \E_{X, \epsilon | \tau} \frac{1}{2} \norm{X\eta - (X\theta_\tau + \epsilon)}_2^2 =  \E_{X, \epsilon | \tau} \frac{1}{2} \norm{X\eta - (X\theta_\tau + \epsilon)}_2^2\\
    &= \E_{X, \epsilon | \tau} \frac{1}{2} \paren{(\eta - \theta_\tau)^T X^TX (\eta - \theta_\tau) - 2 (\eta - \theta_\tau)^T X^T \epsilon  + \epsilon^2} \\
    &= \frac{1}{2} \paren{(\eta - \theta_\tau)^T \Sigma_\tau  (\eta - \theta_\tau) + \sigma^2_\tau} \\
    &= \frac{1}{2} \eta^T \Sigma_\tau \eta + \frac{1}{2} \theta_\tau ^T \Sigma_\tau \theta_\tau - \theta_\tau ^T \Sigma_\tau \eta    + \frac{1}{2} \sigma^2_\tau
\end{align*}
where as the empirical risk on a sample $S_\tau=(\bX_s, \by_s)$ of size $n$ is given by:
\begin{align*}
\calR(\eta; S_\tau)  = \frac{1}{n} \norm{\bX_s\eta - \by_s}_2^2
\end{align*}
For initialization based approaches like MAML, the objective is to learn an initialization whose optimal value $\theta^*_{ML}(\alpha)$ is given by: 
\begin{align}
    \arg\min_{\theta} F(\theta) \coloneqq \E_\tau \E_{S_\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; S_\tau) ; \tau) \label{eq:ML-optimal}
\end{align}
which essentially means that, $\theta^*_{ML}(\alpha)$ is an initialization where performing one step of gradient descent on a support set $S_\tau$ of size $n$, for a task sampled from the meta-distribution $p(\tau)$, achieves the minimal total risk. 

\underline{Fix-Support Meta-Learning:} If the task distribution is given by $p(\tau)$ we define the true risk for parameter $\eta$ on task $\tau$ with fixed support $\bX_F$ as $\calR(\eta; \bX_F, \tau)$:

\begin{align*}
    \calR(\eta; \bX_F, \tau) &= \E_{y | \bX_F, \tau} \frac{1}{2} \norm{\bX_F\eta - y}_2^2 = \E_{\epsilon | \tau} \frac{1}{2} \norm{\bX_F\eta - (\bX_F\theta_\tau + \epsilon)}_2^2 \\
    & =  \E_{\epsilon | \tau} \frac{1}{2} \norm{\bX_F\eta - (\bX_F\theta_\tau + \epsilon)}_2^2\\
    &= \E_{\epsilon | \tau} \frac{1}{2} \paren{(\eta - \theta_\tau)^T X_F^TX_F (\eta - \theta_\tau) - 2 (\eta - \theta_\tau)^T X_F^T \epsilon  + \epsilon^2} \\
    &= \frac{1}{2} \paren{(\eta - \theta_\tau)^T \bX_F^T \bX_F  (\eta - \theta_\tau) + \sigma^2_\tau} \\
    &= \frac{1}{2} \eta^T \bX_F^T \bX_F \eta + \frac{1}{2} \theta_\tau ^T \bX_F^T \bX_F \theta_\tau - \theta_\tau ^T \bX_F^T \bX_F \eta    + \frac{1}{2} \sigma^2_\tau
\end{align*}
where as the empirical risk on a sample $S_\tau(\bX_F)=(\bX_F, \by_s)$ of size $n$ is given by:
\begin{align*}
\calR(\eta; S_\tau(\bX_F))  = \frac{1}{n} \norm{\bX_F\eta - \by_s}_2^2
\end{align*}
% For initialization based approaches like MAML, the objective is to learn an initialization whose optimal value $\theta^*_{ML}(\alpha)$ is given by: 
% \begin{align*}
%     \arg\min_{\theta} \E_\tau \E_{S_\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; S_\tau) ; \tau)
% \end{align*}
% which essentially means that, $\theta^*_{ML}(\alpha)$ is an initialization where performing one step of gradient descent on a support set $S_\tau$ of size $n$, for a task sampled from the meta-distribution $p(\tau)$, achieves the minimal total risk. 



\begin{lemma}
If $X \perp \tau$ then the objective fixing a single support $\bX_F$ is optimizing a biased version of the original objective for meta-learning in \eqref{eq:ML-optimal}:
\end{lemma}


\begin{align*}
    \E_\tau \E_{S_\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; S_\tau) ; \tau) 
    &= \E_{\tau} \E_{X,\epsilon|\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; X, \epsilon) ; \tau)\\
    &= \E_{X} \E_{\tau|X} \E_{\epsilon|\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; X, \epsilon) ; \tau)\\
    &= \E_{X} \E_{\tau} \E_{\epsilon|\tau} \calR(\theta - \alpha \nabla_\theta \calR(\theta; X, \epsilon) ; \tau)
\end{align*}

where the last equality is given by the assumption $X \perp \tau$. If for the outermost expectation over $X$, we replace it with a point estimate by fixing $X=\bX_F$, then we recover the \fixml objective in \eqref{eq:FixML-optimal}

% \hline

We shall now derive the optimum parameters $\theta^*_{\textrm{FML}}(\alpha, X_s)$ for a particular value of the fixed support set $X_s$ and $\theta^*_{\textrm{ML}}(\alpha)$ on the  meta task distribution, with the task-specific risk defined as above. 


\begin{align*}
    \theta^*_{\textrm{FML}}(\alpha, X_s) &= \arg\min \E_\tau \brck{\E_{\epsilon_s | \tau} \calR(\hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau);\theta_\tau, \tau)} \\
    \theta^*_{\textrm{ML}}(\alpha) &= \arg\min \E_\tau \brck{\E_{X_s, \epsilon_s | \tau} \calR(\hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau);\theta_\tau, \tau)} \\
    \hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau) &= \theta- \alpha \frac{1}{2}\nabla_\theta \norm{X_s\theta - (X_s\theta_\tau + \epsilon_s)}_2^2 = \theta - \alpha X_s^TX_s (\theta - \theta_\tau) - \alpha X_s^T\epsilon_s 
\end{align*}


% \begin{align*}
%      \E_{\epsilon_s | \tau} \hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau) &= \E_{\epsilon_s | \tau} \brck{\theta - \alpha X_s^TX_s (\theta - \theta_\tau) - \alpha X_s^T\epsilon_s} \\
%     & = \theta - \alpha X_s^TX_s (\theta - \theta_\tau) = (\bI - \alpha X_s^TX_s) \theta + \alpha X_s^TX_s \theta_\tau
% \end{align*}

% \\
%     & = \theta - \alpha X_s^TX_s (\theta - \E_{\tau} \theta_\tau) = (\bI - \alpha X_s^TX_s) \theta + \alpha X_s^TX_s \E_\tau\brck{\theta_\tau}


% \begin{align*}
%   \E_{X_s, \epsilon_s | \tau}  \hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau) &= \E_{X_s, \epsilon_s | \tau} \brck{\theta - \alpha X_s^TX_s (\theta - \theta_\tau) - X_s^T\epsilon_s} \\
%     & = \E_{X_s} \brck{ \theta - \alpha X_s^TX_s (\theta - \theta_\tau)} \\
%     & = \theta - \alpha \Sigma_\tau (\theta - \green{\E_{\tau}} \theta_\tau) = (\bI - \alpha \Sigma_\tau) \theta + \alpha \Sigma_\tau \theta_\tau
% \end{align*}


\begin{lemma}
Given the task distribution $p(\tau)$ and the task specific risk $\calR(\cdot; \theta_\tau, \tau)$ defined as above, the optimal solutions $\theta^*_{\textrm{FML}}(\alpha, X_s)$ and $\theta^*_{\textrm{ML}}(\alpha)$ are given by solving $ \nabla_\theta \E_\tau \brck{\E_{\epsilon_s | \tau} \calR(\hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau);\theta_\tau, \tau)} = 0$ and $\nabla_\theta \E_\tau \brck{\E_{X_s, \epsilon_s | \tau} \calR(\hat{\theta}(X_s, \epsilon_s, \alpha, \theta_\tau);\theta_\tau, \tau)} = 0$ respectively and are given by:
\label{lemma:opt-sol}
\begin{align*}
    \theta^*_{\textrm{FML}}(\alpha, X_s) &= \paren{\paren{\bI - \alpha X_s^TX_s} \E_\tau\brck{\Sigma_\tau} \paren{\bI - \alpha X_s^TX_s}}^{-1} \paren{\E_\tau\brck{\paren{\bI - \alpha X_s^TX_s} \Sigma_\tau \paren{\bI - \alpha X_s^TX_s}\theta_\tau}} \\
    \theta^*_{\textrm{ML}}(\alpha) &= \paren{\E_\tau \E_{\hat{\Sigma}_\tau} \brck{\paren{\bI - \alpha \hat{\Sigma}_\tau} \Sigma_\tau \paren{\bI - \alpha \hat{\Sigma}_\tau}}}^{-1} \paren{\E_\tau \E_{\hat{\Sigma}_\tau} \brck{\paren{\bI - \alpha \hat{\Sigma}_\tau} \Sigma_\tau \paren{\bI - \alpha\hat{\Sigma}_\tau}\theta_\tau}}
\end{align*}
\end{lemma}


If $\theta_\tau \perp \Sigma_\tau, \hat{\Sigma}_\tau$, then the solution is just given by the mean of $\theta_\tau$. The Hessian for the convex quadratic objectives are given by:

\begin{align*}
    \bH_{\textrm{FML}}(\alpha, X_s) &= \paren{\bI - \alpha X_s^TX_s} \E_\tau\brck{\Sigma_\tau} \paren{\bI - \alpha X_s^TX_s} \\
    \bH_{\textrm{ML}}(\alpha) &= \E_\tau \E_{\hat{\Sigma}_\tau} \brck{\paren{\bI - \alpha \hat{\Sigma}_\tau} \Sigma_\tau \paren{\bI - \alpha \hat{\Sigma}_\tau}}
\end{align*}

Here, $\hat{\Sigma}_\tau$ is the RV which denotes an estimate of the uncentered co-variance matrix for a task $\tau$ using $n$ support samples from that task $\hat{\Sigma}_\tau = \frac{1}{n} X_s^T X_s$. 



\begin{lemma}
If we observe $M$ tasks with task parameters $\{\theta^i\}_{i \in [M]}$, each with $n$ support samples $\{X_s^i, y_s^i\}_{i\in[M]}$ and $n$ query samples $\{X_q^i, y_q^i\}_{i\in[M]}$ such that $X_s^{i}, X_q^{i},  \in \Real^{n \times p}$  and  $y_s^{i}, y_q^{i},  \in \Real^{n}$ and $y_s^i = X_s^i \theta^i + \epsilon_s^i,\, y_q^i = X_q^i \theta^i + \epsilon_q^i $  then the ML minimizer of the empirical loss $\Tilde{F}(\theta)$ is given by:  
\label{lemma:empirical-sol}
\end{lemma}

\begin{align*}
    &\hat{\theta}_{ML} = \\
    &\paren{\sum_{i\in M} (\bI - \frac{\alpha}{n} {X_s^i}^T {X_s^i}) {X_q^i}^T {X_q^i}  (\bI - \frac{\alpha}{n} {X_s^i}^T {X_s^i}^T)}^{-1}  \paren{\sum_{i\in M} (\bI - \frac{\alpha}{n} {X_s^i}^T {X_s^i}) {X_q^i}^T {X_q^i}  (\bI - \frac{\alpha}{n} {X_s^i}^T {X_s^i})(\theta^i - \frac{\alpha}{n} {X_s^i}^{T} \epsilon_s^{i}) + \epsilon_q^i}
\end{align*}

First, $\hat{\theta}_{ML}$ is \textbf{not} an unbiased estimate of ${\theta^*}_{ML}$. Second, controlling the distribution of eigen values for $\Sigma_\tau$ would be futile in cases when $\alpha$ is small. But, in which cases do we need a large learning rate $\alpha$. $F(\theta)$ is quadratic in $\alpha$,  


\subsection*{Special case analyses over the choice of the fixed support $\bX_F$}

For ease of analysis we shall consider the case when there is no observational noise \ie $\epsilon_{s,i} = \epsilon_{q,i} = \b0$. Furthermore, we shall only consider the case where $X_F^TX_F$ (where $X_F$ is the fixed support) and the task-specific uncentered co-variance $\Sigma_\tau$ are diagonal matrices for every task $\tau$. Let $A_F(\alpha)$ be the diagonal matrix:

\begin{align}
    A_F(\alpha) \coloneqq \bI - \frac{\alpha}{n} X^T_F X_F 
\end{align}

and $\tilde{B}_{F,i}(\alpha)$ and $B_{F,i}(\alpha)$ be defined as follows:
\begin{align}
    % A_F(\alpha) &\coloneqq \bI - \frac{\alpha}{n} X_F^T X_F  \\
    \tilde{B}_{F,i}(\alpha) &\coloneqq \frac{1}{n} A_F(\alpha) X_{q,i}^T X_{q,i} A_F(\alpha) \\
    B_{F,i}(\alpha) &\coloneqq  A_F(\alpha) \Sigma_i A_F(\alpha)
\end{align}
From Lemma~\ref{lemma:opt-sol},~\ref{lemma:empirical-sol} we know that for support and query sets drawn from $m$ random tasks the empirical estimate  $\hat{\theta}(X_F, \alpha)$ and the optimal solution $\theta^*(X_F, \alpha)$ are given by:

\begin{align}
    \hat{\theta}(X_F, \alpha) &= \paren{\sum_{i\in[m]} \tilde{B}_{F,i}(\alpha)}^{+} \paren{\sum_{i\in[m]} \tilde{B}_{F,i}(\alpha) \theta_i} \\
    \theta^*(X_F, \alpha) &=  \paren{\E_{\tau} \E_{X_{q}|\tau} \brck{ \tilde{B}_{F,\tau}(\alpha)}}^{+} \paren{\E_{\tau} \E_{X_{q}|\tau} \brck{\tilde{B}_{F,\tau}(\alpha) \theta_\tau}} \\
    &= \paren{\E_{\tau} \brck{{B}_{F,\tau}(\alpha)}}^{+} \E_{\tau}  \brck{{B}_{F,\tau}(\alpha) \theta_\tau}
\end{align}


\begin{lemma}
When we restrict $X_F$ to be a diagonal matrix along with the diagonal task-specific uncentered co-variance matrix $\Sigma_\tau \succ 0$, then we have the following co-ordinate wise closed form solution for $\theta^*(X_F, \alpha)$
\begin{align}
    \theta^*(X_F, \alpha)^{j} &= \frac{\paren{A_F(\alpha)^{j}}^2 \E_\tau\brck{\Sigma_\tau^{(j)} \theta^{j}_\tau}}{
    \paren{A_F(\alpha)^{j}}^2 \E_\tau\brck{\Sigma_\tau^{j}}}  \\
    &= \frac{\E_\tau\brck{\Sigma_\tau^{j} \theta^{j}}}{
     \E_\tau\brck{\Sigma_\tau^{j}}} 
\end{align}
\end{lemma}





\begin{itemize}
    \item In this special case we arrive at the conclusion for fixed $X_F$, as long as $A_F(\alpha) \succ 0$ and diagonal the optimal solution has the exact same value.
    % , since $\theta^*(X_F, \alpha)$ in the above result is not dependent on $X_F$.
    \item This entails that as long as the fixed support $X_F$ satisfies the above conditions, the optimal solution would have the same meta-test performance based on $\norm{\theta^*(X_F, \alpha) - \theta^*( \alpha)}$.
    % we fix they would have the same bias. 
    \item But the variance $\V\brck{\hat{\theta}(X_F, \alpha)}$ of these estimates may differ based on $X_F$ and same for the bias $\norm{\E\brck{\hat{\theta}(X_F, \alpha)}- \theta^*(X_F, \alpha)}$.
\end{itemize}

In expectation over the sampled dataset $\calD$, if we look at the performance of the \fixml solution compared to the best fixed parameter: $\E_\calD \E_\tau \calR(\hat{\theta}(X_F, \alpha);\tau) - \E_\tau \calR(\theta^*( \alpha);\tau)$:

\begin{align}
    & \E_\calD \E_{\tau} \E_{S,Q|\tau} \| \hat{\theta}(X_F, \alpha) - \theta_\tau\|_{\bI - \alpha X_s^T X_s}
    -  \E_{\tau} \E_{S,Q|\tau} \| \theta^*(\alpha) - \theta_\tau\|_{\bI - \alpha X_s^T X_s} \\
    &\leq \E_{\tau} \E_{S,Q|\tau}  \E_\calD \|\hat{\theta}(X_F, \alpha) - \theta^*(\alpha) \|_{\bI - \alpha X_s^T X_s}
\end{align}


Thus, we now try to upper bound $\E_\calD \|\hat{\theta}(X_F, \alpha) - \theta^*(\alpha) \|^2_2$ in the parameter space which breaks down into:

\begin{align}
    \E_\calD \|\hat{\theta}(X_F, \alpha) - \theta^*(\alpha) \|^2_2 = \|\E_\calD \hat{\theta}(X_F, \alpha) - \theta^*(\alpha) \|^2 + \textrm{tr}\paren{\V_\calD \brck{\hat{\theta}(X_F, \alpha)}}
\end{align}


% Thus, we are now interested in this quantity:

% \begin{align}
%     \V\brck{\hat{\theta}(X_F, \alpha)} = \V\brck{\paren{\sum_i \tilde{B}_{F,i}(\alpha)}^{+} \paren{\sum_i \tilde{B}_{F,i}(\alpha) \theta_i}}
% \end{align}


% The other term that we need to analyze is the performance of $ \theta^*(X_F, \alpha)$ compared to the optimal ML solution:


% \begin{align}
%   \abs{F(\theta^*(X_F, \alpha)) - F(\theta^*(\alpha))} 
%   \leq \mu \|\theta^*(X_F, \alpha)) - \theta^*(\alpha)\|_2
%     % \E\abs{F(\hat{\theta}(X_F, \alpha)) - F(\theta^*(\alpha))} 
% %   \leq \mu \|\theta^*(X_F, \alpha)) - \theta^*(\alpha)\|_2^2
% \end{align}



\begin{lemma}
For a query matrix $X_{q,\tau} \in \Real^{n \times p}$ (from task $\tau$) with mean centered rows $X_{q, \tau}^{i}$ satisfying the distributional properties:  $X_{q, \tau}^{i} $ follows a Sub-Gaussian distribution with parameter $\sigma^2$ and $\V\brck{X_{q, \tau}^{i}} = \Sigma_\tau$. Then for some finite constant $C > 0$ we have the following bound on co-variance estimation with probability at least $1 - \delta$
\begin{align}
    \norm{\frac{1}{n} {X_{q, \tau}^{i}}^T X_{q, \tau}^{i} - \Sigma_\tau}  &\leq C \sigma^2 \paren{\sqrt{\frac{p+\log{(2/\delta)}}{n}} + \frac{p+\log{(2/\delta)}}{n}} 
    % &=  \norm{\frac{1}{n} A_F(\alpha) \paren{{X_{q, \tau}^{(i)}}^T X_{q, \tau}^{(i)} - \Sigma_\tau} A_F(\alpha) } \\
\end{align}

\textbf{In our case:} We consider a fixed diagonal matrix $X_F^TX_F$ and $A_F(\alpha)= \textrm{diag}(A_F(\alpha)^{i})$ and diagonal co-variance matrices $\Sigma_\tau =  \textrm{diag}(\Sigma_\tau^{i})$. 
% This implies that task query points $X_{q, \tau}^{i} \in \Real^p$  are co-ordinate wise Sub-Gaussian with parameter $\Sigma_\tau^{j}$ for $X_{q, \tau}^{i,j}$.

\begin{align}
        \norm{\frac{1}{n} A_F(\alpha) \paren{{X_{q, \tau}^{(i)}}^T X_{q, \tau}^{(i)} - \Sigma_\tau}A_F(\alpha)}  &\leq  C' \sigma^2_{F} (\alpha) \paren{\sqrt{\frac{p+\log{(2/\delta)}}{n}} + \frac{p+\log{(2/\delta)}}{n}} \\
        \sigma^2_F(\alpha) &=  \max_i  \Sigma_\tau^i (A_F(\alpha)^i)^2
\end{align}

\end{lemma}



\begin{lemma}
From the matrix Bernstein inequality we can upper bound the spectral norm for the sum of independent random centered matrices. If $\norm{{B}_{F,\tau}(\alpha) - \E_\tau \brck{ {B}_{F,\tau}(\alpha)}} \leq \kappa$, then with probability at least $1-\rho$,
\begin{align}
    \norm{\frac{1}{m}\sum_{i \in [m]} \paren{{B}_{F,i}(\alpha) - \E_\tau \brck{B_{F,\tau}(\alpha)}} } \leq \frac{2\kappa}{3m} \log{(2p/\rho)} + \sqrt{\frac{2\log{(2p/\rho)} \|\V_\tau\brck{B_{F,\tau}(\alpha)}\|}{m}}
\end{align}



% \begin{lemma} 
\textbf{In our case:} The variance $\V_\tau\brck{B_{F,\tau}(\alpha)}$ for a fixed diagonal matrix $X_F^TX_F$, $A_F(\alpha)= \textrm{diag}(A_F(\alpha)^{i})$ and diagonal co-variance matrices $\Sigma_\tau=\textrm{diag}(\Sigma_\tau^{i})$:
\begin{align}
   \sqrt{ \|\V_\tau\brck{B_{F,\tau}(\alpha)}\|} = \max_{i}\paren{{A_F^i(\alpha)}^2\sqrt{\V_\tau\brck{\Sigma_\tau^{i}}}}
\end{align}

\end{lemma}
% \end{lemma}s



\begin{lemma}
From the matrix Chernoff bound we can lower bound the minimum eigen value for the sum of independent random positive semi-definite matrices. If $\|\tilde{B}_{F,i}(\alpha)\|\leq L$ and $\mu_{\min} = \lambda_{\min}( \E_\tau\brck{{B}_{F,\tau}(\alpha)})$, then with probability at least $1-p\paren{\frac{e^{-\epsilon}}{(1-e)^{-\epsilon}}}^{\mu_{\min}/L}$,
\begin{align}
    \lambda_{\min} \paren{\sum_i \tilde{B}_{F,i}(\alpha)} \geq (1-\epsilon) m\mu_{\min}
\end{align}
The minimum eigen value $\lambda_{\min}( \E\brck{{B}_{F,\tau}(\alpha)})$ for a fixed diagonal matrix $X_F^TX_F$, $A_F(\alpha)= \textrm{diag}(A_F(\alpha)^{i})$ and diagonal uncentered co-variance matrices $\Sigma_\tau$:
\begin{align}
    \lambda_{\min}( \E_\tau\brck{{B}_{F,\tau}(\alpha)}) = \min_{i} {A_F(\alpha)^{i}}^2 \paren{\E_\tau\brck{\Sigma_\tau^{i}}}
\end{align}
\end{lemma}


\textbf{Now using the lemmas above, we shall bound the estimation error suffered by fixing a specific support matrix $X_F$.
}
\begin{align}
\hat{\theta}(X_F, \alpha) - \theta^*(\alpha) &= \paren{\sum_i \tilde{B}_{F,i}(\alpha)}^{+} \paren{\sum_i \tilde{B}_{F,i}(\alpha) \theta_i} -\theta^*(\alpha) \nonumber \\
\hat{\theta}(X_F, \alpha) - \theta^*(\alpha)  &= \paren{\sum_i \tilde{B}_{F,i}(\alpha)}^{+} \paren{\sum_i \tilde{B}_{F,i}(\alpha) \paren{\theta_i -\theta^*(\alpha)}}  \nonumber \\
\norm{\hat{\theta}(X_F, \alpha) - \theta^*(\alpha)} &\leq \frac{\norm{\sum_i \tilde{B}_{F,i}(\alpha) (\theta_i - \theta^*(\alpha))}}{\lambda_{\min}\paren{\sum_i \tilde{B}_{F,i}(\alpha)}}
\end{align}

\begin{align}
& \frac{1}{m}\norm{\sum_{i \in [m]} \tilde{B}_{F,i}(\alpha) (\theta_i - \theta^*(\alpha))} \leq  \underbrace{\norm{\frac{1}{m}\sum_{i \in [m]} \paren{\tilde{B}_{F,i}(\alpha) - B_{F,i}(\alpha)} (\theta_i - \theta^*(\alpha))}}_{T_1}  \nonumber \\
& \qquad\qquad  +\underbrace{ \norm{   \frac{1}{m}  \sum_{i \in [m]}  \paren{B_{F,i}(\alpha) - \E_\tau\brck{B_{F,\tau}(\alpha)}} (\theta_i - \theta^*(\alpha))}}_{T_2}\nonumber 
 + \underbrace{\norm{ \E_\tau\brck{B_{F,\tau}(\alpha)} (\theta_i - \theta^*(\alpha))}}_{T_3} 
\end{align}

Each of the three terms on the right can be individually bounded above using the lemmas introduced just before. For $T1$ we apply the union bound over the $m$ observed tasks and with probability at least $1-\delta$:


\begin{align}
    T_1 &\leq  \frac{1}{m} \sum_{i \in [m]} \norm{\tilde{B}_{F,i}(\alpha) - B_{F,i}(\alpha)} \norm{\theta_i -\theta^*(\alpha)} \\
    &\leq   \frac{1}{m} \sum_{i \in [m]} \paren{\Sigma_\tau^i (A_F(\alpha)^i)^2}
    \paren{\sqrt{\frac{p+\log{(2m/\delta)}}{n}} + \frac{p+\log{(2m/\delta)}}{n}} \\
    &\leq \kappa_1 \paren{\sqrt{\frac{p+\log{(2m/\delta)}}{n}} + \frac{p+\log{(2m/\delta)}}{n}} 
\end{align}


\begin{align}
    T_3 &\leq  \kappa_1 \sup_\tau \|\theta_\tau - \theta^*(\alpha)\|  
\end{align}


For $T_2$ we apply the union bound once again to arrive at: with probability atleast $1-\rho$:



\begin{align}
    T_2 &\leq  \frac{2\kappa}{3m} \log{(2p/\rho)} + \sqrt{\frac{2\log{(2p/\rho)} \|\V_\tau\brck{B_{F,\tau}(\alpha)}\|}{m}} \paren{\sup_\tau \|\theta_\tau - \theta^*(\alpha)\|}
\end{align}

So the objective of solving for the best $X_F$ and consequently $A_F$ which minimizes the high probability upper bound reduces to the following \textit{very} simple optimization problem:

\begin{align}
    & \min_{\{A_F^i(\alpha)\}_{i=1}^n} \sup_{i} A_F^i(\alpha)^2 \sqrt{\V\brck{\Sigma_\tau^i}} 
    \qquad \textrm{s.t.} \qquad   A_F^i(\alpha)^2 \E_\tau\brck{\Sigma_\tau^i} \geq \kappa_2 \,\, \forall \tau,i \\
    & \implies A_F^{i*}(\alpha) = \sqrt{\frac{\kappa_2}{\E_\tau\brck{\Sigma_\tau^i}}} 
\end{align}


In the more general case, the optimization problem is given by:

\begin{align}
    & \min_{A_F(\alpha)} \sup \sqrt{\norm{ \V_\tau\brck{{A_F(\alpha) \Sigma_\tau A_F(\alpha)}}}} 
    \qquad \textrm{s.t.} \qquad \kappa_1  \geq  \|A_F(\alpha) \E_\tau\brck{\Sigma_\tau} A_F(\alpha)\| \geq \kappa_2 
\end{align}

% Since $\E \brck{\tilde{B}_{F,i}(\alpha) - {B}_{F,i}(\alpha)} = 0$ and $\norm{\tilde{B}_{F,i}(\alpha) - {B}_{F,i}(\alpha)} \leq \kappa$, then with probability at least $1-\rho$,
% \begin{align}
%     \norm{\sum_i \paren{\tilde{B}_{F,i}(\alpha) - B_{F,i}(\alpha)} } \leq 
% \end{align}


\red{Based on the analysis above we can construct a meta-task distribution and corresponding fixed support matrix that has lower variance and bias compared to \ml.}

\begin{figure*}[ht]
\label{fig:spectrogram}
    \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/regression/diag-1.png}
    \captionsetup{labelformat=empty}
    \caption*{(a)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/regression/diag-2.png}
    \captionsetup{labelformat=empty}
    \end{minipage}
    \caption{$\alpha=0.5$}
    \label{fig:alpha0.5}
\end{figure*}


\subsection{Next Steps on Analysis}

\begin{itemize}
    \item \textbf{Generic case}: Stability based analysis.
    \item \textbf{Linear Regression}: Asymptotic MSE of \fixml solution vs \ml solution. We know that in this case $\hat{\theta}(X_F, \alpha)$ and $\hat{\theta}(\alpha)$ are asymptotically unbiased. In terms of experiments, what if we match train and test for \fixml? Currently we are not doing this.
\end{itemize}


\subsubsection{Stability based analysis}


\paragraph{Notation.} For a meta-algorithm $\calA:\tau^n \rightarrow \Omega$ that maps $n$ tasks to the parameters of a base-learner $A(\omega):\calZ^m \rightarrow \calH\,, \omega \in \Omega$ which in itself maps $m$ training samples to a hypothesis. We shall denote the dataset with a random fixed support pool $S_{p,0}$ by $\calD_{fml}$ and the meta-learner's dataset with the varying support pools as $\calD_{ml}$. Now, consider two quantities: uniform inner-stability $\Tilde{\beta}$ and uniform outer-stability $\beta$, for both \ml and \fixml.


\begin{align}
    \tilde{\beta}_{fml} &= \sup_{\calD_{fml},S,z} \abs{l(\calA(\calD_{fml})(S), z) - l(\calA(\calD_{fml})(S^{\backslash i}, z))} \\
    \tilde{\beta}_{ml} &= \sup_{\calD_{ml},S,z} \abs{l(\calA(\calD_{ml})(S), z) - l(\calA(\calD_{ml})(S^{\backslash i}, z))} \\
    \beta_{fml} &= \sup_{\calD_{fml},S,z} \abs{l(\calA(\calD_{fml})(S), z) - l(\calA(\calD_{fml}^{\backslash i})(S), z)} \\
    \beta_{ml} &= \sup_{\calD_{ml},S,z} \abs{l(\calA(\calD_{ml})(S), z) - l(\calA(\calD_{ml}^{\backslash i})(S), z)} 
\end{align}


\begin{align}
&\abs{\hat{\E}_\tau \hat{\calR}_\tau(\calA(\calD_{fml})(S_{p,0}^\tau)) - \E_\tau \E_{S|\tau} \calR_\tau(\calA(\calD_{fml})(S))} \nonumber \\
&\leq \underbrace{\abs{\hat{\E}_\tau \hat{\calR}_\tau(\calA(\calD_{fml})(S_{p,0}^\tau)) - \hat{\E}_\tau \hat{E}_{S|\tau} \hat{\calR}_\tau(\calA(\calD_{fml})(S))}}_{\textrm{I}} \nonumber \\
&+ \underbrace{\abs{\hat{\E}_\tau \hat{E}_{S|\tau} \hat{\calR}_\tau(\calA(\calD_{fml})(S)) - \E_\tau \E_{S|\tau} \calR_\tau(\calA(\calD_{fml})(S))}}_{\textrm{II}}
\label{eq:genn-gap}
\end{align}

\begin{itemize}
    \item We can verify I from the gap between the blue and red curves for \fixml and \ml. Currently we observe that this gap is much lower for over-parameterized networks.
    \item For II we first apply the bound in Theorem 2 from \cite{chen2020closer} which will allow us to focus on only outer-stability $\beta_{ml}$ and $\beta_{fml}$. \am{The main crux of why II is independent of $\Tilde{\beta}_{*}$ is that in the inner task the support and query is chosen independently and randomly from the task $\tau$ which makes the post-adaptation loss on the query set an unbiased estimate of the generalization gap which $\rightarrow 0$ if  the model is expressive and we train long enough.}
    \item Now, to show that $\beta_{ml}$ has a worst case upper bound compared to the stability of \fixml we need to look at the meta-algorithm learner, which in our case is SGD.
    \item But a distribution independent bound like the one in Theorem 3.10 in \cite{hardt2016train} is not so useful. So we instead need to consider the one in Theorem 2 from \cite{kuzborskij2018data} which shall provide the bound in terms of i) variance of stochastic gradient and ii) curvature at optimization. Note that we have now linked the generalization gap in terms of the variance we observe in terms of optimization, which we know from experiments is lower for \fixml.
    \item To provably show how the outer stability for \fixml has better upper bound we can consider the case of a deep linear network $\bW_0 \cdot \bW_1 \cdot \cdot\cdot  \bW_n (X)$ and a protonet meta-learner for which the analysis of gradient variance is analytically easier to realize.
\end{itemize}



\subsubsection{Asymptotic MSE for Linear Regression}

The MSE for $\hat{\theta}(X_F)$ and $\hat{\theta}$ would concentrate around the AsymMSE at the same rate. \am{And non-asymptotic analysis in the general linear regression case would be a bit tricky here, because of the inverse term. Additionally, having $\Sigma_\tau \not\!\perp\!\!\!\perp \theta_\tau$ would also make the analysis possibly harder. Not sure of the latter.} But for a simpler yet more generic (than the diagonal one) setting we could consider $\Sigma_\tau \perp \theta_\tau$ and $T \rightarrow \infty$.  

\clearpage
\subsection{Empirical Results}


\begin{figure*}[ht]
\label{fig:spectrogram}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=5_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(a)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=10_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(b)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=50_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(c)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=5_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(d)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=10_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(e)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=5_n=50_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(f)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=5_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(g)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=10_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(h)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=50_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(i)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=5_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(j)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=10_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(k)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=10_n=50_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=5_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=10_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=50_p=5_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=5_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=10_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \end{minipage} \hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.5/res_M=50_n=50_p=10_alpha=0.5_n_runs=50.png}
    \captionsetup{labelformat=empty}
    \end{minipage}
    \caption{$\alpha=0.5$}
    \label{fig:alpha0.5}
\end{figure*}






\begin{figure*}[ht]
\label{fig:spectrogram}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=5_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(a)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=10_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(b)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=50_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(c)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=5_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(d)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=10_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(e)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=5_n=50_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(f)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=5_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(g)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=10_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(h)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=50_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(i)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=5_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(j)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=10_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(k)}
    \end{minipage}\hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=10_n=50_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=5_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=10_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=50_p=5_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \caption*{(l)}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=5_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=10_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \end{minipage} \hfill
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/alpha0.75/res_M=50_n=50_p=10_alpha=0.75_n_runs=200.png}
    \captionsetup{labelformat=empty}
    \end{minipage}
    \caption{$\alpha=0.75$}
    \label{fig:alpha0.75}
\end{figure*}



